Making Sense of Dependence: Efficient Black-box Explanations Using Dependence Measure

This paper presents a new efficient black-box attribution method based on Hilbert-Schmidt Independence Criterion (HSIC), a dependence measure based on Reproducing Kernel Hilbert Spaces (RKHS). HSIC measures the dependence between regions of an input image and the output of a model based on kernel embeddings of distributions. It thus provides explanations enriched by RKHS representation capabilities. HSIC can be estimated very efficiently, significantly reducing the computational cost compared to other black-box attribution methods. Our experiments show that HSIC is up to 8 times faster than the previous best black-box attribution methods while being as faithful. Indeed, we improve or match the state-of-the-art of both black-box and white-box attribution methods for several fidelity metrics on Imagenet with various recent model architectures. Importantly, we show that these advances can be transposed to efficiently and faithfully explain object detection models such as YOLOv4. Finally, we extend the traditional attribution methods by proposing a new kernel enabling an ANOVA-like orthogonal decomposition of importance scores based on HSIC, allowing us to evaluate not only the importance of each image patch but also the importance of their pairwise interactions. Our implementation is available at https://github.com/paulnovello/HSIC-Attribution-Method.

==> draft <==
Let $f: [0,2]^3 \rightarrow \{0,1\}$ such that 
$$
\begin{equation*}
       \textnormal{y} = f(x_1, x_2, x_3) = 
   \begin{dcases}
    1 & \text{if  } x_1 \in [0,1], x_2 \in [1,2], x_3 \in [0,1],\\
    1 & \text{if  } x_1 \in [0,1], x_2 \in [0,1], x_3 \in [1,2],\\
    0 & \text{otherwise.  } 
    \end{dcases}
\end{equation*}
$$
The function $f$ is illustrated in Appendix A. Here, $x_i$ is analogous to $M_i$. In that case, it is clear that $x_1$ is important to explain the output. However, assessing the effect of $x_2$ and $x_3$ is more difficult. They are clearly important to explain the output $\textnormal{y}$, but it can be shown theoretically that $HSIC(x_2, \textnormal{y})=0$ and $HSIC(x_3, \textnormal{y})=0$. **This motivates to assess the interactions between input variables**. One way to retrieve the information that $x_2$ and $x_3$ are important is to assess $HSIC( x_{2,3} , \textnormal{y})$, where $x_{2,3} = (x_2,x_3)$

As noticed by Reviewer **eNpV**, one could assess $HSIC( x_{2,3} , \textnormal{y})$ without any constraints on the kernel $k$, and the obtained value for $HSIC( x_{2,3} , \textnormal{y})$ would indeed be $>0$ . However, by doing so, we would also obtain that $HSIC( x_{1,2} , \textnormal{y}) > 0$ and $HSIC( x_{1,3} , \textnormal{y}) > 0$, whereas $x_1$ does not interact with $x_2$ and $x_3$, only because of the individual effect of $x_1$. We empirically illustrate this by assessing these metrics using the estimator of Eq. 2 with $p=10000$, and kernels $k$, $l$ chosen as the Radial Basis Function (RBF). The results are found in Table 1 below and show that:
* $HSIC(x_2, \textnormal{y}) \approx HSIC(x_3, \textnormal{y}) \approx 0$
* $HSIC( x_{1,2} , \textnormal{y}) \approx HSIC( x_{1,3} , \textnormal{y}) > HSIC( x_{2,3}, \textnormal{y})$

| $HSIC(x_1, \textnormal{y})$ | $HSIC(x_2, \textnormal{y})$ | $HSIC(x_2, \textnormal{y})$ | $HSIC( x_{1,3} , \textnormal{y})$ | $HSIC( x_{1,2} , \textnormal{y})$ | $HSIC( x_{2,3} , \textnormal{y})$ |   
| ---------------------------------------- | ---------------------------------------- | ---------------------------------------- | ---------------------------------------------- | ---------------------------------------------- | ---------------------------------------------- | 
| $1.79 \times 10^{-2}$                    | $2.28 \times 10^{-6}$                    | $9.63 \times 10^{-6}$                    | $1.36 \times 10^{-2}$                          | $1.36 \times 10^{-2}$                          | $2.92 \times 10^{-3}$                          |  
**Table 1**: HSIC metrics with $k$ taken as RBF

In order to correctly assess the pairwise interactions of input variables $x_1$ and $x_2$, one has to remove the individual effect of each variable from the $HSIC( x_{1,2} , \textnormal{y})$. The orthogonal decomposition property [1] allows to do so by simply computing $HSIC_{inter}( x_{1,2} , \textnormal{y})$ as

$HSIC_{inter}( x_{1,2} , \textnormal{y}) = HSIC( x_{1,2} , \textnormal{y}) - HSIC(x_1, \textnormal{y}) - HSIC(x_2, \textnormal{y})$

**If the decomposition property does not hold, we are not guaranteed to fully remove the individual effect of $x_1$ and $x_2$** **using the previous formula**. We estimate $HSIC_{inter}( x_{1,2} , \textnormal{y})$ when the kernel $k$ satisfies the decomposition property (in that case, we choose a Sobolev kernel as in [1]), and when it does not, and show that the correct information of  $HSIC_{inter}( x_{1,2} , \textnormal{y})$ is only retrieved when the decomposition property is satisfied. As previously, this is illustrated in the experiment, whose results are found in Table 2. 

|             | $HSIC_{inter}( x_{1,2} , \textnormal{y})$ | $HSIC_{inter}( x_{1,3} , \textnormal{y})$ | $HSIC_{inter}( x_{2,3} , \textnormal{y})$ |
| ----------- | ------------------------------------------------------ | ------------------------------------------------------ | ------------------------------------------------------ |
| $k$ Sobolev | $7.68 \times 10^{-6}$                                  | $2.83 \times 10^{-6}$                                  | $7.85 \times 10^{-4}$                                  |
| $k$ RBF     | $-4.35 \times 10^{-3}$                                 | $-4.30 \times 10^{-3}$                                 | $2.91 \times 10^{-3}$                                                       |
**Table 2**: HSIC metrics for assessing interactions, when $k$ satisfies (Sobolev) / does not satisfy (RBF) the orthogonal decomposition property


In that case, with $k$ satisfying the orthogonal decomposition property (Sobolev), we retrieve that $HSIC_{inter}( x_{1,2} , \textnormal{y}) \approx HSIC_{inter}( x_{1,3} , \textnormal{y}) \approx 0$ and $HSIC_{inter}( x_{2,3} , \textnormal{y})$ is significant. When $k$ does not satisfy the property (RBF), the values are not relevant (a negative value has no meaning since the metric is a distance)
